S0-No-More: A Z-Wave NonceGet Denial of Service Attack utilizing included but offline NodeIDs

In this paper a vulnerability in the Z-Wave protocol specification, especially in the S0 Z-Wave protocol is presented. Devices supporting this standard can be blocked (denial of service) through continuous S0 NonceGet requests. This way a whole network can be blocked if the attacked devices are Z-Wave network controller. This also effects S2 network controller as long as they support S0 NonceGet requests. As only a minimal amount of nonce requests (1 per ~2 seconds) is required to conduct the attack it cannot be prevented by standard countermeasures against jamming.

==> Security analysis report Z-Wave NonceGet Denial of Service attack utilizing included but offline NodeIDs(1)/tikz/attack-sequence-uml.tex <==
\begin{figure}[ht]
 \centering  
  \tikzset{every picture/.append style={transform shape,scale=0.6}} 
  \begin{sequencediagram}
    \newthread[red]{Att}{Attacker impersonated as NodeID 2}
    \newinst[1]{A}{A (NodeID 2, dead)}
    \newthread[gray]{B}{B / Controller (NodeID 1)}
    \newthread{C}{C (NodeID 3, alive)}

    %\begin{sdloop}[green!40]{Run Loop}
    
        \mess{Att}{S0 Nonce Get}{B}
        \mess{B}{Ack}{Att}
        \mess{B}{S0 Nonce Report}{Att}
        \mess{C}{S0 Nonce Get}{B}
        \mess{Att}{S0 Nonce Get}{B}
        \mess{B}{Ack}{Att}
        \mess{B}{S0 Nonce Report}{Att}
        
      %\mess{ctr}{StartCycle}{ss}
      %\begin{call}{ss}{Update()}{ps}{}
      %  \prelevel
      %  \begin{callself}{ctr}{SenseAgent()}{}
      %    \begin{call}[3]{ctr}{Read}{sense}{}
      %    \end{call}
      %  \end{callself}
      %  \prelevel\prelevel\prelevel\prelevel
      %  \setthreadbias{west}
      %  \begin{call}{ps}{PrePhysicsUpdate()}{sense}{}
      %  \end{call}
      %  \setthreadbias{center}
      %  \begin{callself}{ps}{Update()}{}
      %  \end{callself}
      %  \begin{call}{ps}{PostPhysicsUpdate()}{sense}{}
      %  \end{call}
      %\end{call}
      %\mess{ss}{EndCycle}{ctr}
      %\begin{callself}{ctr}{ActAgent()}{}
      %  \begin{call}{ctr}{Write}{sense}{}
      %  \end{call}
      %\end{callself}
    %\end{sdloop}

  \end{sequencediagram}
  \caption{Attack sequence diagram}
  \label{fig:attack_seq_diag}
\end{figure}
